peerRTF: Robust MVDR Beamforming Using Graph Convolutional Network

Accurate and reliable identification of the relative transfer functions (RTFs) between microphones with respect to a desired source is an essential component in the design of microphone array beamformers, specifically when applying the minimum variance distortionless response (MVDR) criterion. Since an accurate estimation of the RTF in a noisy and reverberant environment is a cumbersome task, we aim at leveraging prior knowledge of the acoustic enclosure to robustify the RTFs estimation by learning the RTF manifold. In this paper, we present a novel robust RTF identification method, tested and trained using both real recordings and simulated scenarios, which relies on learning the RTF manifold using a graph convolutional network (GCN) to infer a robust representation of the RTFs in a confined area, and consequently enhance the beamformers performance.

==> notation.tex <==


notation: 

GEVD(eq: 6/7):
$\mathbf{{h}}_{\textrm{GEVD}}(k)$ 

(all microphones)

ifft:
$\mathbf{h}_{\textrm{GEVD}}(k)\longleftrightarrow \mathbf{h}_{\textrm{GEVD,n}}$ 

for each microphone:
${h}_{\textrm{GEVD,n}}^m$

concatenate from $l_{\textrm{non-casual}}$ to $l_{\textrm{casual}}$ in time domain
for each microphone:

$\{{h}_{\textrm{GEVD,n}}^m\}_{n=l_{\textrm{non-casual}}}^{l_{\textrm{casual}}} = \hat{\mathbf{h}}_{\textrm{GEVD}}^m$


frequency domain:

$\hat{\bar{\mathbf{h}}}_{\textrm{GEVD}}^m$

concatenate all M microphones for each frequency(for MVDR):

$\hat{\bar{\mathbf{h}}}_{\textrm{GEVD}}(k)$

$\hat{\bar{\mathbf{h}}}_{\textrm{GCN}}(k)$

$\hat{\bar{\mathbf{h}}}_{\textrm{MP}}(k)$

$\hat{\bar{\mathbf{h}}}_{\textrm{oracle}}(k)$

the notation in the GCN architecture section:

node in the graph:

$\hat{\vect{h}}_{i}$

his neighbors:

$\vect{h}_{i}^{(j)}, j\in\mathcal{N}(i)$

the notation in the Objective functions section:
$\hat{h}_{\textrm{oracle}}^m[n]$

$\hat{h}_{\textrm{GCN}}^m[n]$

in section 2 (problem formulation) it just h(when we define the RTF) 

My suggestion:

The RTF estimate in the frequency domain 
${h}_{\textrm{alg},\ell}^m(k);\;\ell=1,\ldots,{N_{\textrm{train}}},m=0,1,\ldots,M-1,k=0,1,\ldots,K-1$.

The ReIR is obtained by applying \textrm{iFFT}: $\bar{h}_{\textrm{alg},\ell}^m(n);\;\ell=1,\ldots,{N_{\textrm{train}}},m=0,1,\ldots,M-1,n=-n_{\textrm{non-casual}},\ldots,n_{\textrm{casual}}$. 
$n$ is the tap index and not related to the frame indeed $l$, better to change in (1) from $n$ to $t$.

Note the RTF is either obtained from the time domain by an FFT, or directly in the frequency domain and then it is transformed to the time-domain, truncated, and transformed back to the frequency domain. I think there is no need for the non-smoothed RTF, i.e. the one without truncation in the time-domain.

The algorithms are: $\textrm{alg}\in\{\textrm{gevd},\textrm{cln},\textrm{oracle},\textrm{gcn},\textrm{mp}$\}.

Now, we should group them together.


Steering vector:

 $\mathbf{h}_{\textrm{alg},\ell}(k)=\textrm{vec}_m\{{h}_{\textrm{alg},\ell}^m(k)\}$.

and for the feature vectors of the graphs

$\bar{\mathbf{h}}_{\textrm{alg},\ell}^m=\textrm{vec}_n\{\bar{h}_{\textrm{alg},\ell}^m(n)\}$.

Now we have a graph $\bar{\mathcal{H}}^m$ with vertices $\bar{\mathbf{h}}_{\textrm{cln},\ell}^m$ and one $\bar{\mathbf{h}}_{\textrm{gevd},\ell}^m$.


The neighborhood of node $i$:

$\bar{\mathbf{h}}_{\textrm{gevd},i_j}^m, j\in\mathcal{N}(i)$.


